"Don't Downvote A\$\$\$\$\$\$s!!": An Exploration of Reddit's Advice Communities

Advice forums are a crowdsourced way to reinforce cultural norms and moral behavior. Sites like Reddit contain massive amounts of natural language human interaction, with rules and norms unique to each individual subreddit community. To explore this data, we created a dataset with top 1000 posts from each of two such forums, r/AmItheAsshole and r/relationships, and extracted natural language features including sentiment, similarity, word frequency, and demographics using both algorithmic and manual methods. Further, we developed a method to extract demographic information from the subreddits, examined how the post authors' self-disclosures reflect the unique communities in which their posts are shared, and discussed how the authors' language use choices might be related to broader social patterns. We observed some differences between the subreddits in terms of word frequency, demographics disclosure, and gendered language. In general, both subreddits had more female posters than male, and posters tended to use more words about their opposite gender than the same. Gender-diverse posters were uncommon. Implications for future research include a more careful, inclusive focus on identity and disclosure and how that interacts with advice-seeking behavior in online communities.

==> data visualizations/thoughts_on_data_visualizations_-_Kristen.tex <==
Context about this document: This is a place to put assessments about the data visualizations I make

Creator: Kristen Chua

To dos: Help needed described in the PARTS OF SPEECH section

-----------------------------
------ AGE ---------------
-----------------------------
(CURRENT) Count of Posts by Age (2)_June11_newdataset
- Based on dataset advice_subreddits_combined_features_demographics.csv: https://drive.google.com/file/d/1nKfiYbTHgOZhBOkD7-5Zm-nTfHhdfeyD/view?usp=sharing
- Insight: r/AITA is popular among those under 18, r/relationships is  popular to post to among those over 18
https://www.overleaf.com/project/60b80225a354dd82e41823e8(OBSOLETE) Count of posts by age.png 
- Based on dataset subs_combined_sentiment_plus_demographics: https://docs.google.com/spreadsheets/d/1fYX2jIS3F7mjLezCZz2-tgwoZBn6F7PsBxrztriqBfg/edit?usp=sharing

-----------------------------
------ GENDER ---------
-----------------------------
(CURRENT) 
- Based on dataset advice_subreddits_combined_features_demographics.csv: https://drive.google.com/file/d/1nKfiYbTHgOZhBOkD7-5Zm-nTfHhdfeyD/view?usp=sharing
Insight: "n" represents gender nonbinary people
(OBSOLTETE) Count of posts by gender.png
- Based on dataset subs_combined_sentiment_plus_demographics: https://docs.google.com/spreadsheets/d/1fYX2jIS3F7mjLezCZz2-tgwoZBn6F7PsBxrztriqBfg/edit?usp=sharing

---------------------------------
------ SENTIMENT --------
---------------------------------
Count of VADER Compound sentiment values
Insight: The graph is bimodal - its sentiment values frequencies are skewed to the left and right. Used the Gantt view option in Tableau (like a bar chart) to create this graph

-----------------------------------------
----- 	PARTS OF SPEECH -------
-----------------------------------------
AITA & Relationship Verbs & Nouns.xlsx
r AITA & r relationships Noun & Verb groupings.xlsx is a list of tokens I have manually grouped into normalized tokens for the data visualization



Next steps / places where help is needed:
Not capturing compound words too well (example: don't and won't).  Lemmatization issues (it's not cutting up the words right). Classification issues with the NLTK package. Emily helping to create email asking Shiyon, Dr Vick for help as of June 11 2021



https://medium.com/@gianpaul.r/tokenization-and-parts-of-speech-pos-tagging-in-pythons-nltk-library-2d30f70af13b
